Unbiased Learning to Rank: Counterfactual and Online Approaches

This tutorial covers and contrasts the two main methodologies in unbiased Learning to Rank (LTR): Counterfactual LTR and Online LTR. There has long been an interest in LTR from user interactions, however, this form of implicit feedback is very biased. In recent years, unbiased LTR methods have been introduced to remove the effect of different types of bias caused by user-behavior in search. For instance, a well addressed type of bias is position bias: the rank at which a document is displayed heavily affects the interactions it receives. Counterfactual LTR methods deal with such types of bias by learning from historical interactions while correcting for the effect of the explicitly modelled biases. Online LTR does not use an explicit user model, in contrast, it learns through an interactive process where randomized results are displayed to the user. Through randomization the effect of different types of bias can be removed from the learning process. Though both methodologies lead to unbiased LTR, their approaches differ considerably, furthermore, so do their theoretical guarantees, empirical results, effects on the user experience during learning, and applicability. Consequently, for practitioners the choice between the two is very substantial. By providing an overview of both approaches and contrasting them, we aim to provide an essential guide to unbiased LTR so as to aid in understanding and choosing between methodologies.

==> sections/speakers.tex <==
% !TEX root = ../sigir2019-ltr-tutorial-proposal.tex

\section{Detailed Contact Information}
\begin{itemize}
\item \textbf{Harrie Oosterhuis} (main contact person), Informatics Institute, University of Amsterdam, Science Park 904, 1098 XH Amsterdam, The Netherlands. Email: oosterhuis@uva.nl. Telephone: +31 20 525 6786.
\item \textbf{Rolf Jagerman}, Informatics Institute, University of Amsterdam, Science Park 904, 1098 XH Amsterdam, The Netherlands. Email: rolf.jagerman@uva.nl. Telephone: +31 20 525 6786.
\item \textbf{Maarten de Rijke}, Informatics Institute, University of Amsterdam, Science Park 904, 1098 XH Amsterdam, The Netherlands. Email: derijke@uva.nl. Telephone: +31 20 525 5358.
\end{itemize}

\section{Brief Biographies}
\subsection{Harrie Oosterhuis}
Harrie is a third year PhD candidate at the University of Amsterdam under supervision of Professor Dr. Maarten de Rijke.
During his Msc.~in Artificial Intelligence, Harrie completed the Honours program with Cum Laude. Because of this program he already spend two years performing research with Prof.~de Rijke before starting his PhD, resulting in several publications \cite{oosterhuis2016probabilistic, schuth2016multileave, schuth2015probabilistic, oosterhuis2016semantic}.
His main research topics concern user interactions in ranking settings; how to optimize models from such interactions; and how to perform evaluations in these settings. He has multiple publications \cite{li2018optimizing, jagerman2017query, schuth2015probabilistic, schuth2016multileave, oosterhuis2017balancing, oosterhuis2017sensitive, oosterhuis2016probabilistic, oosterhuis2016semantic, oosterhuis2018differentiable, oosterhuis2019optimizing, oosterhuis2018ranking, oosterhuis2018potential} including several on the topic of online learning to rank~\cite{schuth2016multileave, oosterhuis2016probabilistic, oosterhuis2017balancing, oosterhuis2018differentiable, oosterhuis2019optimizing} and reinforcement learning for ranking~\cite{oosterhuis2018ranking}.
Besides academic experience he has industrial experience in the form of three internships at Google research \cite{oosterhuis2016semantic}, one of which concerned reinforcement learning for recommendation.

Harrie has given a four day course on online learning to rank at the 12th Russian Summer School in Information Retrieval~\cite{oosterhuis-2018-online}, this course was also given as a tutorial at the University of Queensland by special request.
Throughout Europe and Australia, for academic and industry audiences he has presented talks on online and counterfactual learning to rank, at Google Inc. in the U.S. he has given lectures on Reinforcement Learning.
At the University of Amsterdam, Harrie has taught the Advanced Information Retrieval course in the MSc. Artificial Intelligence, which focusses on Deep Learning in IR, furthermore, he has given several lectures on Learning to Rank at the MSc. level.

\subsection{Rolf Jagerman}
Rolf is a third year PhD candidate at the University of Amsterdam under supervision of Professor Dr. Maarten de Rijke.
Before joining the University of Amsterdam, Rolf completed his BSc (Cum Laude) at Delft University of Technology and his MSc at ETH Z\"urich.
His main research interests range from counterfactual evaluation and learning to learning to rank.
He has published in the areas of learning to rank~\cite{jagerman2017query,jagerman2017modeling} and counterfactual evaluation \cite{jagerman2019people}.
Furthermore, Rolf has helped organize and run TREC OpenSearch, a learning to rank competition that uses interleaving to evaluate participants rankings with real clicks~\cite{jagerman2017overview,jagerman2018opensearch}.

Rolf has teaching experience at the University of Amsterdam where he helped teach the Information Retrieval 1 course in the MSc. and the Search Engines course in the BSc. He has given several lectures on counterfactual evaluation and learning at the MSc. level.

\subsection{Maarten de Rijke}
Maarten is a University Professor of Artificial Intelligence and Information Retrieval at the University of Amsterdam. Together with a team of PhD students and postdocs he works on problems at the interface of information retrieval and artificial intelligence, including online and offline learning to rank, recommender systems, and conversational agents. Maarten has taught extensively at all levels, from primary school lectures on search engines and recommender systems and public lectures on search engine technology to advanced tutorials aimed at PhD students and researchers. Recent tutorials taught by Maarten include SIGIR 2015, WSDM 2016, RUSSIR 2017.

